Minimal Absent Words on Run-Length Encoded Strings

A string $w$ is called a minimal absent word (MAW) for another string $T$ if $w$ does not occur (as a substring) in $T$ and any proper substring of $w$ occurs in $T$. State-of-the-art data structures for reporting the set $\mathsf{MAW}(T)$ of MAWs from a given string $T$ of length $n$ require $O(n)$ space, can be built in $O(n)$ time, and can report all MAWs in $O(|\mathsf{MAW}(T)|)$ time upon a query. This paper initiates the problem of computing MAWs from a compressed representation of a string. In particular, we focus on the most basic compressed representation of a string, run-length encoding (RLE), which represents each maximal run of the same characters $a$ by $a^p$ where $p$ is the length of the run. Let $m$ be the RLE-size of string $T$. After categorizing the MAWs into five disjoint sets $\mathcal{M}_1$, $\mathcal{M}_2$, $\mathcal{M}_3$, $\mathcal{M}_4$, $\mathcal{M}_5$ using RLE, we present matching upper and lower bounds for the number of MAWs in $\mathcal{M}_i$ for $i = 1,2,4,5$ in terms of RLE-size $m$, except for $\mathcal{M}_3$ whose size is unbounded by $m$. We then present a compact $O(m)$-space data structure that can report all MAWs in optimal $O(|\mathsf{MAW}(T)|)$ time.

==> construction.tex <==
\section{Constructing MAW representations}

In this section we present how to construct our $O(m)$-space
RLE-based representation of all MAWs in $T$.

\begin{lemma} \label{M1_construction}
Given $\rle(T)$ of size $R(T) = m$,
the representation $D_1$ for $\mathcal{M}_1$ can be constructed in $O(m \log m)$ time and $O(m)$ space.
%表現$D_1$は$O(m \log m)$時間で構築可能である.
\end{lemma}
\begin{proof}
  We perform a simple linear scan over $\rle(T)$.
  If $\Sigma'_T$ is an integer alphabet of polynomial size in $m$,
  $D_1$ can be built in $O(m)$ time and space.
  Otherwise, $D_1$ can be built in $O(m + \sigma'_T \log \sigma'_t)$ time
  and $O(\sigma')$ working space.
  Since $\sigma'_T \leq m$ the lemma holds.
%文字列$T$を$O(m)$時間かけて走査し，$T$中の$\sigma'$種類全ての文字に対し，最大の連の長さを記録する．この$\sigma'$個の配列を$\sigma' \log \sigma'$文字の辞書式順序でソートすると，$D_1$を得る．$\sigma' \leq m$より，この構築時間は$O(m \log m)$時間である．
\end{proof}

\begin{lemma} \label{M2_construction}
Given $\rle(T)$ of size $R(T) = m$,
the representation $D_1$ for $\mathcal{M}_1$ can be constructed in $O(m \log m)$ time and $O(m)$ space.
%表現$D_2$は$O(m \log m)$時間で構築可能である.
\end{lemma}
\begin{proof}
  Since $D_2$ is the trie of bigrams occurring in $T$,
  we can incrementally build $D_2$ by scanning $\rle(T)$,
  using $O(m + \sigma'_T \log \sigma'_T) \subseteq O(m \log m)$ and $O(\sigma'_T) \subseteq O(m)$ space.
%文字列$T$を$O(m)$時間かけて走査し，$T$中の2グラム(最大$m-1$種類)全てに対する2グラム木を，辺が辞書式順序を維持するように構築する．$O(m \log \sigma')$時間で$D_2$を得る．$\sigma' \leq m$より，この構築時間は$O(m \log m)$時間である．
\end{proof}

\begin{lemma}
\label{M3_construction}
表現$D_3$は$O(m \log m)$時間で構築可能である.
\end{lemma}
\begin{proof}
文字列$T$を$O(m)$時間かけて走査し，$T$中の3グラム(最大$m-2$種類)全てに対し$S'\alpha$を各$\sigma'$種類の$\alpha$に対し構築する．$O(m \log m)$時間で$S'\alpha$を，$\alpha$の指数でソートする．$O(m \log \sigma')$時間で$\sigma_r, \sigma_l$を得たのち，$O(m \log \sigma')$時間で$Q_r, Q_l$ を得る．$S'_\alpha,Q_r,Q_l$をそれぞれ$\sigma'$種類構築したことにより，$D_3$を得る．$\sigma' \leq m$より，この構築時間は$O(m \log m)$時間である．
\end{proof}

\begin{lemma}
\label{M4_construction}
表現$D_4$は$O(m \log m)$時間で構築可能である.
\end{lemma}
\begin{proof}
$K(\alpha u \beta)$が判明しているならば，二部グラフ$G_{\alpha u \beta}$を構築し，$O(m \log m)$時間で$V_A$と$V_B$を，それぞれ$\alpha, \beta$の指数でソートすることで構築できる．

長さ$O(1)$のブリッジは，文字列を全て走査して$O(m \log m)$時間で列挙できる．しかし，それより長い$\alpha u \beta$については，この方法だとそれぞれ$K(\alpha u \beta)$を$O(m \log m)$時間で得ることになってしまう．

そこで，power reductionを考える．$Y_3$をソートした列を${y_1, \ldots , y_{|Y_3|}}$とする．長さ$m$の文字列$T'$を構築する．
$T'$の全ての位置$s (1 \leq s \leq m)$は以下を満たす．
\begin{itemize}
\item $T$の$s$番目の連の開始位置を$i$，その連の長さを$j$としたとき，$T[i-1.. i+j] = y_k$ならば$T'[s] = k$．
\end{itemize}
このとき，以下が成り立つ．
\begin{observation}
ブリッジ$z = \alpha_0\alpha_1^{p_1} ... \alpha_h^{p_h}\alpha_{h+1}$が$x$番目の連の$1$つ前の位置から始まるとき，$y'_1, \ldots, y'_h = \alpha_0\alpha_1^{p_1}\alpha_2 , \ldots , \alpha_{h-1}\alpha_{h}^{p_h}\alpha_{h+1}$とすると，$T'[x ..x+p-1] = y'_1 \cdots y'_h$
\end{observation}
\begin{lemma}
$T'[x ..x+p-1] = y'_1 \cdots y'_h$ならば，$y'_1, \ldots, y'_h = \alpha_0\alpha_1^{p_1}\alpha_2 , \ldots , \alpha_{h-1}\alpha_{h}^{p_h}\alpha_{h+1}$となる文字$\alpha_0 , \ldots ,  \alpha_{h+1}$と整数$p_1 , \ldots , p_h$が存在して，ブリッジ$z = \alpha_0\alpha_1^{p_1} ... \alpha_h^{p_h}\alpha_{h+1}$が$T$の$x$番目の連の$1$つ前の位置に出現する．
\end{lemma}
\begin{proof}
まず，$y'_{1} = \alpha_{0}\alpha_{1}^{p_1}\alpha_{2}$となる$\alpha_{0},\alpha_{1},\alpha_{2},p_1$を定める．
$y'_i = \alpha_{i-1}\alpha_{i}^{p_i}\alpha_{i+1}$ならば，定義より$y'_{i+1}[1..2] = \alpha_{i}\alpha_{i+1}$であり，$y'_{i+1} = \alpha_{i}\alpha_{i+1}^{p_i}\alpha_{i+2}$となる$\alpha_{i+2},p_i$を定められる．
このとき，$T$の$x+i$番目の連は$\alpha_{i}^{p_i}$である．
\end{proof}

上記の補題により，$T'$で2回以上出現する部分文字列を探すと，それは$T$上での2回以上出現するブリッジであることと同値になる．
よって，$T'$からsuffix Treeを作り，内部ノードを全て列挙し，そこから$K$を得る．二部グラフを得た後のソートは$O(m \log m)$時間である．
\end{proof}

\begin{lemma}
\label{M5_construction}
表現$D_5$は$O(m \log m)$時間で構築可能である.
\end{lemma}
\begin{proof}
$\mathcal{M}_5$に含まれるMAWの列挙と同値である．
$\mathcal{M}_5$に含まれるMAW$aub$を，以下の条件により5つに分ける．
\begin{enumerate}
\item $m' = 2$かつ$1$番目の連の長さが$1$ (Type5-1)
\item $m' = 2$かつ$m'$番目の連の長さが$1$ (Type5-2)
\item $m' \geq 3$かつ$1$番目の連の長さが$1$ (Type5-3)
\item $m' \geq 3$かつ$m'$番目の連の長さが$1$ (Type5-4)
\item $1$番目と$m'$番目の連の長さが$2$以上 (Type5-5) 
\end{enumerate}
以後，証明のため$\alpha, \beta, \gamma$を用いる．それぞれについて，$\alpha \neq \beta ,\beta \neq \gamma ,\gamma \neq \alpha$を仮定する．

Type5-1のMAWは$2 \leq k$となる$k$を用いて$\alpha\beta^k$と表せる．Type4のMAWを列挙する際に用いる二部グラフ$G_{\alpha\beta}$と$\mathcal{M}_1$に含まれる$\beta$のMAW$\beta^{k'}$に対し，以下の補題が成り立つ．
\begin{lemma}
$G_{\alpha\beta}$において，$f_3(|V_B|) = k-1$，かつ$\mathcal{M}_1$に含まれる$\beta$のMAWが$\beta^{k'}(k' > k)$であることは，$\alpha\beta^k$がMAWであることと同値である．
\end{lemma}
\begin{proof}
$A \rightarrow B$を示す．$f_3(|V_B|) = k-1$ならば，グラフの定義より$\alpha\beta^{k-1}$が出現し，$\alpha\beta^k$が出現しない．また，$\mathcal{M}_1$に含まれる$\beta$のMAW$\beta^{k'}$の指数$k'$が$k' > k$ならば$\beta^k$は出現する．よって，$\alpha\beta^k$はMAWである．
次に$B \rightarrow A$を示す．$\alpha\beta^k$がMAWとすると，$f_3(|V_B|) \geq k$ならば，$\alpha\beta^k$は出現する．$f_3(|V_B|) < k-1$ならば，$\alpha\beta^{k-1}$は出現しない．$\mathcal{M}_1$に含まれる$\beta$のMAW$\beta^{k'}$の指数$k'$が$k' \leq k$ならば，$\beta^k$が出現しない．よって，$f_3(|V_B|) = k-1$かつ$\beta^{k'}$の指数$k'$は$k' > k$である．
\end{proof}
Type5-2のMAWも同様に示せる．

Type5-3のMAWは，文字列$u$ ($\epsilon$も可)と，$2 \leq k_1 , 2\leq k_2$となる$k_1k_2$を用いて$\alpha \gamma^{k_1} u\beta^{k_2}$と表せる．ただし，$u[1] \neq \gamma, u[|u|] \neq \beta$である．
二部グラフ$G_{\gamma u \beta}$において，以下の補題が成り立つ．
\begin{lemma}
$G_{\gamma u \beta}$において，$f_1(v_a) = \alpha, f_2(v_a) =k_1$となる頂点$v_a \in V_A$が存在して$ f_3(E_{max}(v_a)) = k_2 - 1$を満たし，かつ$f_3(|V_B|) \geq k_2$であることは，$\alpha \gamma^{k_1} u\beta^{k_2}$がMAWであることと同値である．
\end{lemma}
\begin{proof}
$A \rightarrow B$を示す．$f_1(v_a) = \alpha, f_2(v_a) =k_1, f_3(E_{max}(v_a)) = k_2 - 1$となる頂点$v_a \in V_A$が存在ならば，$\alpha \gamma^{k_1} u\beta^{k_2-1}$が出現し，$\alpha \gamma^{k_1} u\beta^{k_2}$は出現しない．$f_3(|V_B|) \geq k_2$より$\gamma^{k_1} u\beta^{k_2}$が出現するため，$\alpha \gamma^{k_1} u\beta^{k_2}$はMAWである．

次に，$B \rightarrow A$を示す．$\alpha \gamma^{k_1} u\beta^{k_2}$がMAWと仮定する．$f_1(v_a) = \alpha, f_2(v_a) =k_1$となる頂点$v_a \in V_A$が存在しないならば，$\alpha \gamma^{k_1} u\beta$が出現しない．そのような$v_a$が存在しても$ f_3(E_{max}(v_a)) < k_2 - 1$ならば，$\alpha \gamma^{k_1} u\beta^{k_2-1}$が出現しない．逆に，$ f_3(E_{max}(v_a)) < k_2 - 1$ならば，$\alpha \gamma^{k_1} u\beta^{k_2}$が出現する．$f_3(|V_B|) < k_2$ならば，$\gamma^{k_1} u\beta^{k_2}$が出現しない，よって，$\alpha \gamma^{k_1} u\beta^{k_2}$はMAWならば，$f_1(v_a) = \alpha, f_2(v_a) =k_1$となる頂点$v_a \in V_A$が存在して$ f_3(E_{max}(v_a)) = k_2 - 1$を満たし，かつ$f_3(|V_B|) \geq k_2$である．
\end{proof}
Type5-4のMAWも同様に示せる．

Type5-5のMAWは文字列$u$と$2 \leq k_1, 2 \leq k_2$となる$k_1,k_2$を用いて$\alpha^{k_1}u \beta^{k_2}$と表せる．ただし，$u[1] \neq \alpha, u[|u|] \neq \beta$である．Type4のMAWを列挙する際に用いる二部グラフ$G_{\alpha u \beta}$に対し，以下の補題が成り立つ．
\begin{lemma}
$G_{\alpha u \beta}$において，$f_2(|v_a|) \geq k_1, f_3(E_{max}(|v_a|)) = k_2 -1$を満たす$v_a \in V_A$が存在し，かつ$f_3(|v_b|) \geq k_2$を満たす全ての頂点$v_b \in V_B$の$f_2(E_{max}(|v_b|))$の最大値が$k_1-1$であることは，$\alpha^{k_1} u \beta^{k_2}$がMAWであることと同値である．
\end{lemma}
\begin{proof}
$A \rightarrow B$を示す．$f_2(|v_a|) = k_1, f_3(E_{max}(|v_a|)) = k_2 -1$となる頂点$v_a$があるならば，$\alpha^{k_1} u \beta^{k_2-1}$は出現する．$f_3(|v_b|) \geq k_2$を満たす全ての頂点$v_b \in V_B$の$f_2(E_{max}(|v_b|))$の最大値が$k_1-1$ならば，$\alpha^{k_1} u \beta^{k_2}$は出現が出現せず，$\alpha^{k_1-1} u \beta^{k_2}$が出現する．すなわち，$\alpha^{k_1} u \beta^{k_2}$がMAWである ．

次に，$B \rightarrow A$を示す．$\alpha^{k_1} u \beta^{k_2}$がMAWとすると，$f_2(|v_a|) \geq k_1, f_3(E_{max}(|v_a|)) = k_2 -1$となる頂点$v_a$がないならば，$\alpha^{k_1} u \beta^{k_2-1}$が出現しない．$f_3(|v_b|) \geq k_2$を満たす全ての頂点$v_b \in V_B$の$f_2(E_{max}(|v_b|))$の最大値が$k_1 - 1$より大きいならば$\alpha^{k_1} u \beta^{k_2}$が出現し，$k-1 - 1$より小さいならば$\alpha^{k_1 - 1} u \beta^{k_2}$が出現しない．よって，$f_3(|v_b|) \geq k_2$を満たす全ての頂点$v_b \in V_B$の$f_2(E_{max}(|v_b|))$の最大値は$k_1-1$である．
\end{proof}

\end{proof}

\section{補足説明}
\begin{itemize}
\item 岡部くんが示した$\mathcal{M}_4$の上界は，間違っている可能性が高いです (少なくとも，間違っていることが示せる下界を見つけました)．なので，上界は自分が領域を$O(m)$にするために使用した式から示しました．
\item $D_4$の領域の構築が$O(m \log m)$時間になりました．
\end{itemize}

